Semi-Automatically Extracting FAQs to Improve Accessibility of Software Development Knowledge

Frequently asked questions (FAQs) are a popular way to document software development knowledge. As creating such documents is expensive, this paper presents an approach for automatically extracting FAQs from sources of software development discussion, such as mailing lists and Internet forums, by combining techniques of text mining and natural language processing. We apply the approach to popular mailing lists and carry out a survey among software developers to show that it is able to extract high-quality FAQs that may be further improved by experts.

==> unused-text.tex <==
Typically being practical, those pairs are independent and self-contained for the sake of a quick reference to a variety of specific issues.
That is, one does not have to read the whole document to understand a particular answer and usually navigates it through a question index.
Since the FAQ's ultimate goal is to answer the most questions with the least effort on the part of the reader as possible, all questions-answer (Q\&A) pairs ought to be compact and precise.
%The main objective in creating FAQs is to provide quick solutions to a wide range of common questions, such that one does not have to read the whole FAQ to understand a particular answer.
%All questions-answer (Q\&A) pairs ought to be self-contained, compact and precise and are usually grouped by topics.
%Large FAQs usually are browsed through a question index.

%\todo{``What kinds of questions would one expect to find in a
%   FAQ on a particular topic?  How are they normally structured, or are they
%   expected to be searched?  I suspect this varies greatly from FAQ to FAQ,
%   which may make automating their creation quite difficult.''}
%\todo{``Footnote 2 is missing.''}

